Long-term experimental study of price responsive predictive control in a real occupied single-family house with heat pump

The continuous introduction of renewable electricity and increased consumption through electrification of the transport and heating sector challenges grid stability. This study investigates load shifting through demand side management as a solution. We present a four-month experimental study of a low-complexity, hierarchical Model Predictive Control approach for demand side management in a near-zero emission occupied single-family house in Denmark. The control algorithm uses a price signal, weather forecast, a single-zone building model, and a non-linear heat pump efficiency model to generate a space-heating schedule. The weather-compensated, commercial heat pump is made to act smart grid-ready through outdoor temperature input override to enable heat boosting and forced stops to accommodate the heating schedule. The cost reduction from the controller ranged from 2-33% depending on the chosen comfort level. The experiment demonstrates that load shifting is feasible and cost-effective, even without energy storage, and that the current price scheme provides an incentive for Danish end-consumers to shift heating loads. However, issues related to controlling the heat pump through input-manipulation were identified, and the authors propose a more promising path forward involving coordination with manufacturers and regulators to make commercial heat pumps truly smart grid-ready.

==> sections/method/parameter_estimation.tex <==
\section{Parameter Identification}
\label{sec_parameter_est}
\subsection{parameter estimation for house model}
The common room temperature, seen in \eqref{eq_common_Tr} is an average of all room temperatures weighted by the room areas.
\begin{align}
    \label{eq_common_Tr}
    \Tr = \Arj{1}\Tri{1} + \cdots + \Arj{\numRooms}\Tri{\numRooms} 
\end{align}
The identification for the model is performed in two steps, first, a grey-box estimation of the parameters and then a state space sub space method SSID. An advantage of using only two states for the model is that it is possible to solve for the grey-box parameters although they are not given, and thereby anchor the solution physically. The second important signal is the sun irradiation seen in
\begin{align}
    \Isun = \Isundir (1 -\perc_\cloud)
\end{align}
where \Isundir is direct sun $[W/m^2]$ and $\perc_\cloud$ is the fraction of cloud cover. This particular formulation gives short but intense bursts of sunlight. This lets the model partly express the rapid changes to air temperature which the direct sunlight can cause.
%\subsection{Parameters identification for photovoltaic model}
%\subsection{Parameters identification for heat pump model}




\begin{itemize}
    \item externalities 
\end{itemize}

==> sections/results/cop_behavior.tex <==
% \subsection{COP distribution}
% \begin{figure}[H]
% 	\centering
% 	%\includegraphics[width=.7\columnwidth]{figs/dQ_fit.pdf}
% 	\includegraphics[width=1\columnwidth]{figs/dummy_cop_behavior.pdf}
% 	\label{fig_cop_behavior_fit}
% 	\caption{}
% \end{figure}
